Target-Aware Generative Augmentations for Single-Shot Adaptation

In this paper, we address the problem of adapting models from a source domain to a target domain, a task that has become increasingly important due to the brittle generalization of deep neural networks. While several test-time adaptation techniques have emerged, they typically rely on synthetic toolbox data augmentations in cases of limited target data availability. We consider the challenging setting of single-shot adaptation and explore the design of augmentation strategies. We argue that augmentations utilized by existing methods are insufficient to handle large distribution shifts, and hence propose a new approach SiSTA, which first fine-tunes a generative model from the source domain using a single-shot target, and then employs novel sampling strategies for curating synthetic target data. Using experiments on a variety of benchmarks, distribution shifts and image corruptions, we find that SiSTA produces significantly improved generalization over existing baselines in face attribute detection and multi-class object recognition. Furthermore, SiSTA performs competitively to models obtained by training on larger target datasets. Our codes can be accessed at https://github.com/Rakshith-2905/SiSTA.

==> sections/related.tex <==
\section{Related Works}
\label{sec:related}
The problem of distribution shift 
\begin{itemize}
    \item Image space augmentation based techniques
    \item Feature space augmentation
\end{itemize}

\textbf{GAN based domain adaptation:}
    \cite{morerio2020generative} deploys a conditional GAN trained on target dataset with noisy pseudo labels generated by the source model to generate clean target distribution. Approaches like \cite{sankaranarayanan2018generate} \cite{hu2018duplex} \cite{hoffman2018cycada} aims at bringing the source and target distribution closer in a learned joint feature space, such methods depend on the availability of both source and target distribution. Few GAN-based strategies \cite{gal2021stylegan} \cite{zhu2021mind} have been proposed for few-shot domain adaptation tasks, both of these solutions utilize CLIP a multi-modal(language and visual) encoder to model the domain gap.  \cite{yang2020one} proposes 

==> sections/table.tex <==
\begin{table*}[t]
\label{tab:results}
\renewcommand{\arraystretch}{1.3}
\small
\centering
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{clcccclcccc}

\cline{1-1} \cline{3-6} \cline{8-11}
\multicolumn{1}{|c|}{\cellcolor[HTML]{00009B}{\color[HTML]{FFFFFF} }}                                   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{4}{c|}{\cellcolor[HTML]{00009B}{\color[HTML]{FFFFFF} \textbf{Attribute: Smiling}}}                                                                                                                                                                                                                                                   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{4}{c|}{\cellcolor[HTML]{00009B}{\color[HTML]{FFFFFF} \textbf{Attribute: Gender}}}                                                                                                                                                                          \\ \cline{3-6} \cline{8-11} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{00009B}{\color[HTML]{FFFFFF} \textbf{Methods}}}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Domain A}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Domain B}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Domain C}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Average}}                      & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Domain A}} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Domain B}} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Domain C}}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Average}}     \\ \cline{1-1} \cline{3-6} \cline{8-11} 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} Source only}}                        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{89.78}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 73.68}}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 62.18}}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 75.21}}          & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}94.47}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}83.72}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}69.43}                & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}82.54}                \\ \cline{1-1} \cline{3-6} \cline{8-11} 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} MEMO (AugMix)}}                      & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \ul{89.34}}}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 71.76}}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 59.43}}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 73.51}}          & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}94.04}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}82.45}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}58.51}                & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}78.33}                \\ \cline{1-1} \cline{3-6} \cline{8-11} 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} MEMO (RandConv)}}                    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} {\ul 89.37}}}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 71.80}}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 59.27}}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 73.48}}          & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}94.05}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}82.45}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}58.76}                & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}78.42}                \\ \cline{1-1} \cline{3-6} \cline{8-11} 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} Ours (base)}}                        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 84.80}}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 82.53}}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} {83.29}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 83.54}}          & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{94.73}}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\ul 87.52}}       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}89.44}                & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}90.56}                \\ \cline{1-1} \cline{3-6} \cline{8-11} 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} Ours (prune-zero)}}                & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} {88.65}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{85.75}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} {\ul 85.89}}}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{86.76}}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{94.75}}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.03}}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{ \textbf{93.49}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.42}}       \\ \cline{1-1} \cline{3-6} \cline{8-11} 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} Ours (prune-rewind)}}              & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} { 87.63}}}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} {\ul 83.13}}}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{85.99}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} {\ul 85.58}}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\ul 94.68}}       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{ 86.38}}       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\ul {93.18}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\ul 91.41}}          \\ \cline{1-1} \cline{3-6} \cline{8-11} 
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} Oracle}}                             & \multicolumn{1}{l|}{\multirow{-9}{*}{\cellcolor[HTML]{FFFFFF}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} 92.34}}          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} 87.92}}          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} 88.80}}          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} 89.69}}          & \multicolumn{1}{l|}{\multirow{-9}{*}{\cellcolor[HTML]{FFFFFF}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}96.91}             & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}92.13}             & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}95.42}                & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}94.82}                \\ \cline{1-1} \cline{3-6} \cline{8-11} 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{11}{l}{\cellcolor[HTML]{FFFFFF}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             \\ \cline{1-1} \cline{3-6} \cline{8-11} 
\rowcolor[HTML]{00009B} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{00009B}{\color[HTML]{FFFFFF} }}                                   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{4}{c|}{\cellcolor[HTML]{00009B}{\color[HTML]{FFFFFF} \textbf{Attribute: Arched Eyebrows}}}                                                                                                                                                                                                                                           & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{4}{c|}{\cellcolor[HTML]{00009B}{\color[HTML]{FFFFFF} \textbf{Attribute: Mouth Slightly Open}}}                                                                                                                                                             \\ \cline{3-6} \cline{8-11} 
\rowcolor[HTML]{DAE8FC} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{00009B}{\color[HTML]{FFFFFF} \textbf{Methods}}}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Domain A}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Domain B}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Domain C}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Average}}                      & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Domain A}} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Domain B}} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Domain C}}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Average}}     \\ \cline{1-1} \cline{3-6} \cline{8-11} 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}Source only}                                               & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}72.94}                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}51.29}                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}56.71}                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}60.31}                                 & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}88.24}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}80.36}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}60.61}                & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}76.40}                \\ \cline{1-1} \cline{3-6} \cline{8-11} 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}MEMO (AugMix)}                                             & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}72.72}                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}51.23}                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}56.38}                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}60.11}                                 & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}88.22}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}80.30}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}60.60}                & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}76.37}                \\ \cline{1-1} \cline{3-6} \cline{8-11} 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}MEMO (RandConv)}                                           & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}72.66}                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}51.26}                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}56.44}                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}60.12}                                 & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}88.11}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}80.27}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}60.49}                & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}76.29}                \\ \cline{1-1} \cline{3-6} \cline{8-11} 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}Ours (base)}                                               & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}76.39}                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}73.57}                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\ul {65.37}}}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}71.78}                                 & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}91.07}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}82.49}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}69.84}                & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}81.13}                \\ \cline{1-1} \cline{3-6} \cline{8-11} 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}Ours (prune-zero)}                                       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.23}}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{74.41}}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}63.57}                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\ul {72.40}}}                  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.36}}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{84.75}}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\ul 73.31}}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\ul {83.47}}} \\ \cline{1-1} \cline{3-6} \cline{8-11} 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}Ours (prune-rewind)}                                     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\ul 78.26}}                           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\ul 73.91}}                           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{69.68}}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{73.95}}                        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\ul 91.72}}       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\ul 83.11}}       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{77.22}}       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{84.02}}       \\ \cline{1-1} \cline{3-6} \cline{8-11} 
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}Oracle}                                                    & \multicolumn{1}{l|}{\multirow{-9}{*}{\cellcolor[HTML]{FFFFFF}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}81.85}                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}72.94}                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}80.09}                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}78.29}                                 & \multicolumn{1}{l|}{\multirow{-9}{*}{\cellcolor[HTML]{FFFFFF}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}92.94}             & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}88.39}             & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}87.78}                & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}89.70}                \\ \cline{1-1} \cline{3-6} \cline{8-11} 
\end{tabular}
}

\caption{\textbf{Domain-aware augmentation significantly improves generalization.} We report the single-shot SFDA performance (Accuracy \%) across different face attribute detection tasks and domain shifts. \alg~consistently improves upon MEMO while also performing competitively to the oracle. Through \textbf{bold} and \underline{underline} formatting, we denote the top two performing methods.}
\end{table*}

==> sections/temp.tex <==
The performance of deep learning models can suffer greatly when the assumption that the training (source) and target data are from the same distribution is violated. To mitigate this test-time adaptation emerged as a solution where, a source data trained model is adapted to test data with a distribution shift in a few steps using an unsupervised objective.  However, realizing effective test time adaptation under severely limited data setting is very challenging. Traditionally, it has been found that the generality of source representations plays an important role in effective target domain adaptation. Recent techniques rely on upgrading the source model using domain invariant datasets to pave the way for such representations. This has been achieved through Generative image translation techniques

This has been achieved through the use of mix-up techniques between the source data and generic representations, generative image translation techniques between different domains, and classic image augmentation techniques including randconv and augmix.  However, such strategies need a source-level update as well as target adaptation on a substantial dataset.  

In this paper, we investigate the possibility of deriving generic representations from extremely restricted target data without altering the source model. On this front, we propose that generative augmentations can be a potential solution to this problem. Although generative augmentation-based approaches have been utilized in the past, their effectiveness in producing generic representations is dependent on the exposure of the generative models to substantial quantity of data from multiple domains. 
This greatly diminishes the use of such approaches in situations where obtaining multidomain data distributions is not viable. Taking these constraints into consideration, we investigate a more realistic situation in which we must build target - aware domain invariant representations with very few shots at test time. Our method builds upon the ability of state-of-the-art generative models like StyleGAN in order to synthetically expand the target dataset using a single example without human supervision either by labeling the target sample or pre-specifying domain-specific prior knowledge. 

Our approach is comprised of two steps, 1) Synthetic data generation, where we adapt the StyleGAN to the target domain using a single target example which enables us to generate a rich synthetic target domain dataset by sampling in the StyleGANs latent space. To additionally improve the transfer of source knowledge to the target model we introduce different GAN manipulation techniques like systematic activation pruning and weights rewinding that generates images along the geodesic of the source and the target domain. 2) We utilize the state-of-the-art unlabeled source-free unsupervised domain adaptation technique namely NRC in order to adapt the predictive model trained on the source data using only the synthetic samples.

Although approximating the complete target distribution by exposing the generative model to a single target picture is not straightforward, we discover that they learn several important modes of the target distribution, allowing sampling along the geodesic between the source and the target distribution. 

